Stable super-resolution limit and smallest singular value of restricted Fourier matrices

We consider the inverse problem of recovering the locations and amplitudes of a collection of point sources represented as a discrete measure, given $M+1$ of its noisy low-frequency Fourier coefficients. Super-resolution refers to a stable recovery when the distance $\Delta$ between the two closest point sources is less than $1/M$. We introduce a clumps model where the point sources are closely spaced within several clumps. Under this assumption, we derive a non-asymptotic lower bound for the minimum singular value of a Vandermonde matrix whose nodes are determined by the point sources. Our estimate is given as a weighted $\ell^2$ sum, where each term only depends on the configuration of each individual clump. The main novelty is that our lower bound obtains an exact dependence on the {\it Super-Resolution Factor} $SRF=(M\Delta)^{-1}$. As noise level increases, the {\it sensitivity of the noise-space correlation function in the MUSIC algorithm} degrades according to a power law in $SRF$ where the exponent depends on the cardinality of the largest clump. Numerical experiments validate our theoretical bounds for the minimum singular value and the sensitivity of MUSIC. We also provide lower and upper bounds for a min-max error of super-resolution for the grid model, which in turn is closely related to the minimum singular value of Vandermonde matrices.

==> commentout.tex <==
%% commentout
\commentout{
% % % % % % % % % % % % % % % % % % % %
\section{Duality and Interpolation}
\label{sec:preliminaries}



\commentout{
% % % % % % % % % % % % % % % % % % % %
\subsection{Notation}

The symbols $M,S,\mu,\Omega,\omega_j,\eta,\delta,\Phi,x,y$ always refer to the objects defined in the introduction. We also reserve $W,L$ for other objects that we shall define later. Many of these depend on the model parameters, but we suppress their dependence for ease of notation, since the model parameters are fixed throughout.

, so Generic constants are typically written as $C,C_1,C_2$, and if a constant depends on particular quantities, then the dependences are usually made explicit. For other generic objects, we use $\mu$ for measures, $f,g,h,F,G,H$ for functions, $t$ for a real variable, $u,v$ for vectors, $P,Q,R$ for integers, $j,k,m,n$ for indices, and $\alpha,\beta,\gamma,\varphi$ as parameters. 

The one-dimensional torus group is denoted $\T=\R/\Z$. For a non-negative real number $a$, let $|a|_\T$ be the distance between $a$ and the closest integer. We shall also deal with some number theoretic issues. Let $\lfloor a\rfloor$ and $\lceil a\rceil$ be the standard floor and ceiling functions, respectively. For any $a\geq 1$, let $r(a)=a/\lfloor a\rfloor$ and note that $r(a)\geq 1$ with $r(a)=1$ if and only if $a$ is an integer. 

Let $M(\T)$ be the set of bounded Radon measures on $\T$. We write $\delta_a$ to denote the Dirac measure supported at $a\in\T$. For integers $m$ and $n$, the quantity $\delta_{m,n}$ is defined to be $1$ if $m=n$ and be to $0$ if $m\not=n$. Let $L^p(\T)$ for $0<p\leq \infty$ be the usual Lebesgue spaces with norm $\|\cdot\|_{L^p}$. The (unitary) Fourier transform of $\mu\in M(\T)$ and $f\in L^1(\T)$ are denoted $\hat\mu$ and $\hat f$, respectively. 

Let $\C^N$ be the space of $N$-dimensional complex vectors and $\C^N_S$ be the subset of vectors that have at most $S$ non-zero components. For a vector $u\in\C^N$, let $\|u\|_0$ be the number of non-zero entries in $u$, $\|u\|_2$ be its Euclidean norm, and $\supp(u)$ be the subset of $\{0,1,\dots,N-1\}$ for which $u$ is non-zero on. For a complex matrix $X$, its Hermitian transpose is denoted $X^*$ and its Moore-Penrose psuedoinverse is denoted $X^\dagger$.
}


% % % % % % % % % % % % % % % % % % % %
\subsection{Duality}

Our method for estimating $\sigma_{\min}(\Phi)$ is through a dual characterization. We begin with some notation and definitions. Let $\P(M)$ be the space of all smooth functions $f$ on $\T$ of the form  
\[
f(\omega)=\sum_{m=0}^{M} \hat f(m)e^{2\pi im\omega}.
\]
We call $f$ a {\it trigonometric polynomial} of degree at most $M$. 

\begin{definition}[Polynomial interpolation set]
	Given $\Omega=\{\omega_j\}_{j=1}^S\subset\T$ and $u\in\C^S$, the polynomial interpolation set, denoted by $\P(\Omega,M,u)$, is the set of $f\in\P(M)$ such that $f(\omega_j)=u_j$ for each $1\leq j\leq S$. 
\end{definition}

In this definition, we think of $u$ as a function from $\Omega$ to $\C$. The polynomial interpolation set is non-empty whenever $S\leq M-1$. Indeed, recall that the {\it Lagrange polynomials} adapted to $\Omega$ is the set of functions $\{L_j\}_{j=1}^S$, where
\[
L_j(\omega)
=L_j(\omega,\Omega)
=\prod_{k\not=j} \frac{e^{2\pi i\omega}-e^{2\pi i\omega_k}}{e^{2\pi i\omega_j}-e^{2\pi i\omega_k}}.
\]
We readily verify that for any $u\in\C^S$, if we define the function $L$ by the formula,
\[
L(\omega)=L(\omega,\Omega,u)=\sum_{j=1}^S u_jL_j(\omega),
\]
then $L\in\P(\Omega,S-1,u)$. This is usually called the {\it Lagrange interpolant} of $u$. 

\begin{proposition}[Exact duality]
	\label{prop:duality}
	Fix positive integers $M$ and $S$ such that $S\leq M-1$. For any set $\Omega=\{\omega_j\}_{j=1}^S\subset\T$, let $\Phi=\Phi(\Omega,M)$ be the $(M+1)\times S$ Vandermonde matrix associated with $\Omega$ and $M$. If $\sigma_{\min}(\Phi)=\|\Phi u\|_2$ for some unit norm vector $u\in\C^S$, then
	\[
	\sigma_{\min}(\Phi)
	=\max_{f\in \mathcal{P}(M,\Omega,u)} \|f\|_{L^2(\T)}^{-1}.
	\]
\end{proposition} 

\begin{proof}
	The set of all trigonometric polynomials $f\in\P(M)$ can be written in the form 
	\[
	f(\omega)
	=\sum_{m=0}^{M-1} \hat f(m) e^{2\pi i m\omega}.
	\]
	Then $f\in \P(M,\Omega,u)$ if and only if $f\in\P(M)$ and it Fourier coefficients satisfy the under-determined system of equations,
	\[
	u_j
	=\sum_{m=0}^{M-1} \hat f(m) e^{2\pi im\omega_j}
	\quad\text{for}\quad
	1\leq j\leq S.
	\]
	By our earlier observation about the Lagrange polynomials, there exists a $f\in\P(\Omega,M,u)$. Since $\|f\|_{L^2(\T)}=\|\hat f\|_{\ell^2(\Z)}$, the functions $f\in\P(M)$ that satisfy this system of equations and have minimal $L^2(\T)$ norm are the ones with Fourier coefficients given by the Moore-Penrose inverse. Namely,
	\[
	\min_{f\in \P(M,\Omega,v)} \|f\|_{L^2(\T)}
	=\min_{\Phi^*v=u} \|v\|_2
	=\|(\Phi^*)^\dagger u\|_2
	=\frac{1}{\sigma_{\min}(\Phi)}.
	\]
	Rearranging this inequality completes the proof of the proposition.
\end{proof}

Proposition \ref{prop:duality} is well-known for the special case that $M-1=S$. Indeed, if $M-1=S$, then $\Phi$ is a square Vandermonde matrix, and for each $u\in\C^S$, the Lagrange interpolant of $u$ is the unique polynomial in $\P(\Omega,S-1,u)$. For the general case that $M\geq S+1$, we suspect that this proposition had been previously discovered, but we are unable to find a reference. Perhaps we could not find the proposition in the literature because, for the following reasons, it is not immediately clear that this result is actually useful for estimating $\sigma_{\min}(\Phi)$. 
\begin{enumerate}[(a)]
	\item 
	In the extreme case that $S\ll M$, we expect $\P(\Omega,M,u)$ to contain a rich set of functions. However, we do not know much about this set, aside from it being convex. Moreover, this set is extremely dependent on $\Omega$ because we know that $\sigma_{\min}(\Phi)$ is highly sensitive to the configuration of $\Omega$. 
	\item 
	We certainly do not know what the right singular vectors of $\Phi$ are. Yet, in order to invoke the duality result, we must examine the set $\P(\Omega,M,u)$, where $u$ is the right singular vector corresponding to $\sigma_{\min}(\Phi)$! 
\end{enumerate}

It turns out that we can circumvent both of these issues, but doing so will introduce additional technicalities and difficulties. We first present a relaxed version of exact duality, which will provide us with an extra bit of flexibility.   

\begin{proposition}[Robust duality]
	\label{prop:duality2}
	Fix positive integers $M$ and $S$ such that $S\leq M$. For any set $\Omega=\{\omega_j\}_{j=1}^S\subset\T$, unit norm vector $u\in\C^S$, and $\epsilon\in\C^S$ with $\|\epsilon\|_2< 1$, if there exists $f\in\P(M)$ such that $f(\omega_j)=u_j+\epsilon_j$ for each $1\leq j\leq S$, then 
	\[
	\|\Phi u\|_2
	\geq (1-\|\epsilon\|_2) \|f\|_{L^2(\T)}^{-1}.
	\]
\end{proposition}

\begin{proof}
	Define the measure $\mu=\sum_{j=1}^S u_j\delta_{\omega_j}$, and note that $\hat\mu(m)=(\Phi u)_m$. We have
	\[
	\Big|\int_{\T} \overline f\ d\mu\Big|
	=\Big|\sum_{j=1}^S \overline{f(\omega_j)} u_j \Big|
	=\Big|\|u\|_2^2+ \sum_{j=1}^S \overline{u_j} \epsilon_j\Big|
	\geq \|u\|_2^2-\|u\|_2\|\epsilon\|_2
	=1-\|\epsilon\|_2. 
	\]
	On the other hand, using that $f\in\P(M)$, Cauchy-Schwartz, and Parseval,
	\[
	\Big|\int_{\T} \overline f\ d\mu\Big|
	=\Big|\sum_{m=1}^{M-1} \overline{\hat f(m)}\hat\mu(m)\Big| 
	\leq \|\hat f\|_{\ell^2(\Z)}\|\Phi u\|_2
	=\|f\|_{L^2(\T)} \|\Phi u\|_2. 
	\]
	Combining the previous two inequalities completes the proof.
\end{proof}

% % % % % % % % % % % % % % % % % % % %
\subsection{Polynomial interpolation}

Exact duality connects the singular values of Vandermonde matrices to interpolation by trigonometric polynomials. For the moment, suppose $\Omega$ consists of just two points that are separated by at least $1/M$. To interpolate a given $u\colon\Omega\to\C$, we can use a function with good localization properties. For a positive integer $P$, the normalized {\it Fej\'er kernel}, $F_P\in C^\infty(\T)$, is defined by the formula,
\[
F_P(\omega)
=\frac{1}{P+1}\sum_{m=-P}^P \(1-\frac{|m|}{P+1}\) e^{2\pi im\omega}
=\frac{1}{(P+1)^2} \(\frac{\sin(\pi (P+1)\omega)}{\sin(\pi \omega)}\)^2. 
\]
The normalization is chosen so that $F_P(0)=1$. 

We recall some basic facts about the Fej\'er kernel. Its $L^2(\T)$ norm can be calculated using Parseval's formula, and so
\[
\|F_P\|_{L^2(\T)}
=\frac{1}{(P+1)^2}\((P+1)^2+2\sum_{m=1}^P m^2\)^{1/2}
\leq \frac{1}{(P+1)^{1/2}}. 
\]
We can also provide a point-wise estimate. By the trigonometric identity $|\sin(\pi \omega)|\geq 2|\omega|_\T$, we have
\[
|F_P(\omega)|\leq \frac{1}{2^2(P+1)^2|\omega|_\T^2},
\quad\text{for all}\quad
\omega\in \T.
\]
If we raise the Fej\'er kernel to a power $R$, then the function $(F_P(\omega))^R$ has better decay, but at the cost of increasing its frequency support. If we keep the product $PR$ fixed, then increasing $R$ leads to better decay at the expense of worse localization near the origin.

However, if $\Omega$ consists of just two points that are separated by some distance that is smaller than $1/M$. In this case, the Fej\'er kernel fails to provide good interpolation because it is well-localized in an interval whose length exceeds $1/M$ provided that $P\leq M/2$. Thus, how do we interpolate points that are closer than the Rayleigh length? This effect is not specific to the Fej\'er kernel, since Tur\'an \cite{turan1946rational} proved the following result that applies to all trigonometric polynomials.

\begin{proposition}
	If $f\in\P(M)$, $\|f\|_{L^\infty(\T)}=1$, $|f(0)|=1$, and $f(\alpha)=0$, then we necessarily have $\alpha\geq 1/(2M)$. Moreover, equality is achieved by the functions $f(\omega)=c(1+e^{2\pi iM\omega})/2$, where $c$ is uni-modular.
\end{proposition} 

At a first glance, Tur\'an's theorem seems to imply that the interpolation of two points whose distance is much smaller than the Rayleigh length is impossible, but that is not true. For example, for any $\alpha\in\T$, consider the function
\[
f(\omega)=\frac{e^{2\pi i \omega}-e^{2\pi i\alpha}}{1-e^{2\pi i\alpha}},
\]
which satisfies $f(0)=1$ and $f(\alpha)=0$. This does not contradict Tur\'an's theorem because $\|f\|_{L^\infty(\T)}$ is large whenever $|\alpha|_\T$ is small. Instead, Tu\'an's theorem tells us that we must pay a price, in the $L^\infty(\T)$ norm, for interpolating points below the Rayleigh length. 

We can generalize this example to other Lagrange-like polynomials. For convenience, we define the subset,
\[
\Gamma_j
=\Gamma_j(\Omega,M)
=\Big\{\omega_k\in \Omega\colon |\omega_j-\omega_k|_\T< \frac{1}{M}\Big\}.
\]
We call this the {\it cluster centered at $\omega_j$}. If $\omega_j$ is the only element of $\Gamma_j$, then we say it is an {\it isolated point}; otherwise, we say $\omega_j$ is a {\it cluster point}. For convenience, we let 
\[
\gamma_j=\gamma_j(M,\Omega)=|\Gamma_j|,
\]
which is the number of points in the $j$-th cluster. We shall use polynomials of the form (as well as variations of this polynomial), 
\[
W_j(\omega)
=W_j(\omega,\Omega,M)
=\prod_{\omega_k\in \Gamma_j\setminus\{\omega_j\}} \frac{e^{2\pi i P_{j,k}t}-e^{2\pi i P_{j,k}\omega_k}}{e^{2\pi i P_{j,k}\omega_j}-e^{2\pi i P_{j,k}\omega_k}},
\]
where the integers $P_{j,k}$ will be appropriately depending on the intended application. We see that 
\[
W_j(\omega_k)=\delta_{j,k},
\quad\text{for all}\quad
\omega_k\in\Gamma_j.
\]
In general, $W_j$ does not enjoy any good localization properties, so its $L^\infty(\T)$ and $L^2(\T)$ norms are similar. 

By Tur\'an's theorem, the $L^\infty(\T)$ of $W_j$ should be large if $\Gamma_j$ contains many closely spaced points, which is the case. If we start with the inequality,
\[
\|W_j\|_{L^\infty(\T)}
\leq \prod_{\omega_k\in \Gamma_j\setminus\{\omega_j\}} \frac{2}{|1-e^{2\pi i P_{j,k}(\omega_j-\omega_k)}|},
\]
then the right hand side is large if $P_{j,k}\omega_j$ and $P_{j,k}\omega_k$ are close together. Hence, the ``game" is to choose the integers $P_{j,k}$ so that they are as far apart as possible, under the constraint that the degree of $W_j$ does not exceed $M$. Our construction of $W_j$ was inspired by uniform dilation problems on the torus, which was studied and applied to number theory in \cite{alon1992uniform,konyagin2000uniformly}.

In the process of quantifying the norm of these polynomials, we discovered the following notion. We define the {\it complexity} $\rho_j$ of $\omega_j$ in the following way. If $\omega_j$ is an isolated point, we define $\rho_j=1$. If $\omega_j$ is a cluster point, then let
\begin{equation}
	\label{eq:complexity}
	\rho_j
	=\rho_j(\Omega,M)
	=\prod_{\omega_k\in \Gamma_j\setminus\{\omega_j\}} \frac{\gamma_j}{\pi M|\omega_j-\omega_k|_\T}.
\end{equation}
It follows from this definition that $\rho_j=1$ if and only if $\omega_j$ is an isolated point and $\rho_j>1$ otherwise. The ratio $M/\gamma_j$ is the average local over-sampling ratio because we there are $M+1$ Fourier samples and $\gamma_j$ points in the $j$-th cluster. The $\pi$ factor comes from the fact that $2\pi|\omega_j-\omega_k|_\T$ is approximately $|e^{2\pi i\omega_j}-e^{2\pi i\omega_k}|$ when $M$ is large. 

The complexity varies greatly depending on the exact structure of $\Gamma_j$. It is large if $\Gamma_j$ consists of many points. It can be as small as a constant, if $|\omega_j-\omega_k|_\T$ is about $1/M$ for each $\omega_k\in \Gamma_j\setminus\{\omega_j\}$. On the other hand, it can be significantly larger than $M$, if for example, there are two points in $\Gamma_j$ that are separated by $1/M^2$. While the complexity captures our intuition for how dense a cluster is, we shall see that it mathematically quantifies a $L^\infty(\T)$ penalty incurred for interpolating points within a Rayleigh length. 

% % % % % % % % % % % % % % % % % % % %
\subsection{TV min vs. subspace methods}

Total variation minimization is a completely different approach for estimating the measure $\mu$ from the measurements $y$. The papers in this community usually assume we are given $2m+1$ consecutive Fourier samples. To compare their setting with ours, we assume throughout this section that $2m\approx M$. Note that the Rayleigh length is $1/(2m)\approx 1/M$.

In the noiseless setting, the standard convex approach is to solve the {\it total variation minimization} (TV-min) problem: Given the noiseless Fourier measurements $y\in\C^{2m+1}$ of some unknown measure $\mu\in M(\T)$, find the solution(s) $\nu\in M(\T)$ to 
\begin{equation}
\tag{TV}
\label{TV}
\min_\nu  \|\nu\|_{TV}
\quad\text{such that}\quad
y_m = \hat\nu(m)
\quad\text{for}\quad
m=0,1,\dots,M-1.
\end{equation}
This method dates back to some classical work of Beurling \cite{beurling1989balayage,beurling1989interpolation}, and there has been renewed interest in this problem, see \cite{candes2013super,fernandez2013support,tang2015near,azais2015spike,morgenshtern2016super,li2017elementary,benedetto2018super}. 

Even in the noiseless setting, without additional assumptions on the discrete measure $\mu$, the Dirac masses must be separated by at least $1/m$, approximately twice the Rayleigh length. To make this statement precise, we say a discrete set $\Omega\subset\T$ satisfies the {\it TV-min uniform recovery property} if any complex valued measure $\mu$ supported in $\Omega$ is the unique solution to \eqref{TV} given its first $2m+1$ Fourier coefficients. Then we recall the following facts, which can be found in \cite{fernandez2016super,da2018tight}.

\begin{proposition}
	If $m\geq 10^3$ and $\Delta(\Omega)\geq 1.26/m$, then $\Omega$ satisfies the TV-min uniform recovery property. On the other hand, if $m$ is sufficiently large and $\Omega$ satisfies the TV-min uniform recovery property, then $\Delta(\Omega)\geq 1/m-O(1/m^2)$. 
\end{proposition}

\begin{remark}
	We caution the reader that it is still possible to recover certain types of $\mu$ that are not supported in $\Omega$ satisfying the TV-min uniform recovery property. This can happen if the sign of $\mu$ and its support satisfy special properties. For instance, \eqref{TV} can recover positive discrete measures regardless of separation \cite{de2012exact,morgenshtern2016super,denoyelle2017support} and any complex measure with certain sign patterns \cite{benedetto2018super}. 
\end{remark}

Why does (\ref{TV}) require separation in the noiseless case while subspace methods do not? In a nutshell, TV minimization depends on the phase of $x$, the coefficients of the discrete measure $\mu$, whereas subspace methods do not. The following well-known duality can be found in  \cite{candes2014towards,duval2015exact}. 

\begin{proposition}
	Fix a positive integer $m$ and a set $\Omega=\{\omega_j\}_{j=1}^S\subset \T$. Then $\Omega$ satisfies the TV-min uniform recovery problem if and only if for any $u\in\C^S$ with $|u_j|=1$ for each $1\leq j\leq S$, there exists a trigonometric polynomial $f\in\P(2m)$ such that $f(\omega_j)=u_j$ and $f'(\omega_j)=0$ for each $1\leq j\leq S$. 
\end{proposition} 

Hence, the necessary and sufficient condition that $\Omega$ satisfies the uniform TV-min recovery is that for any uni-modular $u\in\C^S$ defined on $\Omega$, there exists a $f$ that solves a Hermite interpolation problem. However, this $f$ does not always exit, if $\Omega$ contains too many closely spaced points, which was the argument given in \cite{da2018tight}. 

On the other hand, subspace methods only depend on the column span of $\calH(y^0)$. Provided that $\Phi_L$ and $\Phi_{M-L}$ have full column rank, which holds if $M-L\geq S+1$ and $L\geq S+1$, the column span of $\calH(y^0)$ coincides with that of $\Phi_L$ via the relationship,
\[
\calH(y^0)=\Phi_L X \Phi_{M-L}.
\]
Recall that $X$ is the diagonal matrix consisting of the $x_j$. This shows that changing the phase of each $x_j$ does not change the column span of $\Phi_L$. This invariance to the phases of $x$ is why subspace methods do not require separation, in the noiseless case. 
}
